Scheduling Bag-of-Tasks in Clouds using Spot and Burstable Virtual Machines

Leading Cloud providers offer several types of Virtual Machines (VMs) in diverse contract models, with different guarantees in terms of availability and reliability. Among them, the most popular contract models are the on-demand and the spot models. In the former, on-demand VMs are allocated for a fixed cost per time unit, and their availability is ensured during the whole execution. On the other hand, in the spot market, VMs are offered with a huge discount when compared to the on-demand VMs, but their availability fluctuates according to the cloud's current demand that can terminate or hibernate a spot VM at any time. Furthermore, in order to cope with workload variations, cloud providers have also introduced the concept of burstable VMs which are able to burst up their respective baseline CPU performance during a limited period of time with an up to 20% discount when compared to an equivalent non-burstable on-demand VMs. In the current work, we present the Burst Hibernation-Aware Dynamic Scheduler (Burst-HADS), a framework that schedules and executes tasks of Bag-of-Tasks applications with deadline constraints by exploiting spot and on-demand burstable VMs, aiming at minimizing both the monetary cost and the execution time. Based on ILS metaheuristics, Burst-HADS defines an initial scheduling map of tasks to VMs which can then be dynamically altered by migrating tasks of a hibernated spot VM or by performing work-stealing when VMs become idle. Performance results on Amazon EC2 cloud with different applications show that, when compared to a solution that uses only regular on-demand instances, Burst-HADS reduces the monetary cost of the execution and meet the application deadline even in scenarios with high spot hibernation rates. It also reduces the total execution time when compared to a solution that uses only spot and non-burstable on-demand instances.

==> draft.tex <==

% \begin{table*}[htb]
% \caption{Execution of  Burst-HADS in scenarios $sc_0$ to $sc_5$. The table shows the average number of hibernations and resume, the  number of used on-demand VMs, the average makespan, the average monetary cost and the percentage difference in makespan and cost compared to the solution that uses only on-demand VMs\label{tab:result}}
% \centering
% \begin{tabular}{ccccccccc}
% \toprule
% \textbf{JOB}          & \textbf{scenario} & \textbf{\# hibernation} & \textbf{\# resume} & \textbf{\# on-demand} & \textbf{makespan}    & \textbf{cost}        & \textbf{makespan  (\%) diff} & \textbf{cost (\%) diff} \\
% \midrule

% \multirow{6}{*}{J60}  & $sc_0$  & 0.00   & 0.00    & 0.00    & 1274  & \$0.112              & -35.39\%                           & 58.72\%                      \\
%                       & $sc_1$  & 0.67   & 0.00    & 0.67    & 1277  & \$0.119              & -35.75\%                           & 56.06\%                      \\
%                       & $sc_2$  & 5.33   & 0.00    & 2.67    & 1752  & \$0.241              & -86.19\%                           & 10.98\%                      \\
%                       & $sc_3$  & 1.33   & 1.33   & 1.33     & 1218  & \$0.128              & -29.40\%                           & 52.95\%                      \\
%                       & $sc_4$  & 4.67   & 4.67   & 1.67     & 1445  & \$0.142              & -53.52\%                           & 47.44\%                      \\
%                       & $sc_5$  & 2.67   & 0.00   & 2.00     & 1408  & \$0.176              & -49.63\%                           & 35.15\%                      \\
%                       \cline{2 - 9}
                      
% \multirow{6}{*}{J80}  & $sc_0$  & 0.00   & 0.00   & 0.00     & 1171  & \$0.133              & 6.94\%                             & 57.37\%                      \\
%                       & $sc_1$  & 1.33   & 0.00   & 1.33     & 1419  & \$0.167              & -12.77\%                           & 46.36\%                      \\
%                       & $sc_2$  & 5.33   & 0.00   & 2.00     & 2267  & \$0.258              & -80.21\%                           & 17.09\%                      \\
%                       & $sc_3$  & 0.67   & 0.67   & 0.67     & 1367  & \$0.164              & -8.66\%                            & 47.50\%                      \\
%                       & $sc_4$  & 8.00   & 8.00   & 3.00     & 2488  & \$0.244              & -97.75\%                           & 21.57\%                      \\
%                       & $sc_5$  & 3.67   & 2.33   & 3.00     & 1589  & \$0.195              & -26.34\%                           & 37.37\%                      \\
%                       \cline{2 - 9}
% \multirow{6}{*}{J100} & $sc_0$  & 0.00   & 0.00   & 0.00     & 1660  & \$0.176              & -13.54\%                           & 52.63\%                      \\
%                       & $sc_1$  & 1.33   & 0.00   & 1.00     & 1798  & \$0.230              & -22.96\%                           & 37.94\%                      \\
%                       & $sc_2$  & 4.00   & 0.00   & 2.33     & 1900  & \$0.279              & -29.96\%                           & 24.72\%                      \\
%                       & $sc_3$  & 3.00   & 2.00   & 1.67     & 1925  & \$0.237              & -31.65\%                           & 36.15\%                      \\
%                       & $sc_4$  & 8.33   & 7.00   & 5.00     & 2553  & \$0.328              & -74.65\%                           & 11.62\%                      \\
%                       & $sc_5$  &        &        &          &       &                      &                                    & \\
%                       \cline{2 - 9}
% \multirow{6}{*}{J200} & $sc_0$  &     & &  &  & &  & \\
%                       & $sc_1$  &     & &  &  & &  & \\
%                       & $sc_2$  &     & &  &  & &  & \\
%                       & $sc_3$  &     & &  &  & &  & \\
%                       & $sc_4$  &     & &  &  & &  & \\
%                       & $sc_5$  &     & &  &  & &  & \\


%                       \bottomrule

% \end{tabular}
% \end{table*}



% In Amazon Elastic Compute Cloud (EC2),  users have two main options of instance's contracting model: the  {\it on-demand} and the  {\it spot} market. While the on-demand market has plenty of guarantees in terms of reliability,  the spot one offers unused resources for a lower price without such guarantees. Thus, despite the monetary advantages,  a spot instance can be terminated or hibernated by EC2 at any moment.  Moreover, different instance types are offered by  EC2 with variations in terms of computational resources, price, and optimizations to fit different use cases. One of those types is the general-purpose burstable instances. Those instances are offered at a low price on the on-demand market (when compared to other instances with the same capacities) and have the ability to burst to high levels of CPU utilization as long the user has enough CPU credits. Therefore, on-demand burstable instances have all the guarantees offered by the on-demand market but need constant management of CPU credits and CPU utilization, which adds more complexity to the scheduling problem on cloud environments. Thus, in this work, we propose the burst-HADS an extended version of the Hibernation-Aware Dynamic Scheduler (HADS) that combines spot and burstable instances to schedule bag-of-tasks application subjected to a deadline constraint. Our practical results show that, when compared to a solution that uses only regular on-demand instances, burst-HADS was able to reduce the monetary cost of the execution and meet the deadline even in scenarios with high spot revocations rate (hibernations). Moreover, the results also showed that burst-HADS also reduces the total execution time (makespan) when compared to the HADS first version, showing  that combining spot and on-demand burstable instances have the  potential not only to minimize the monetary cost but also
